A Correctness Result for Synthesizing Plans With Loops in Stochastic Domains

Finite-state controllers (FSCs), such as plans with loops, are powerful and compact representations of action selection widely used in robotics, video games and logistics. There has been steady progress on synthesizing FSCs in deterministic environments, but the algorithmic machinery needed for lifting such techniques to stochastic environments is not yet fully understood. While the derivation of FSCs has received some attention in the context of discounted expected reward measures, they are often solved approximately and/or without correctness guarantees. In essence, that makes it difficult to analyze fundamental concerns such as: do all paths terminate, and do the majority of paths reach a goal state? In this paper, we present new theoretical results on a generic technique for synthesizing FSCs in stochastic environments, allowing for highly granular specifications on termination and goal satisfaction.

==> incubator.tex <==
This implies that an action with multiple outcomes doesn't reduce the likelihood of a run, so when the planner synthesises a controller for an environment, it is either correct or not correct; there is no middle ground, such as a likelihood of partial correctness.


The AND-steps perform the depth-first search among controllers, using the partial ordering $\prec$, and the OR-steps perform the depth-first search in the controller histories.


==> sec-conclusion.tex <==
\section{Conclusion}

To conclude, this paper was motivated by FSCs, which are powerful and compact representations for action selection. We presented new algorithmic foundations for synthesizing FSCs in stochastic environments, by means of a probabilistic extension of the AND-OR schema. It allows for highly granular specifications, and is provably correct, which we think is significant for safety-critical applications, among others.  Understanding and comparing the benefits of this approach to others based on discounted expected reward measures is one possible direction for the future, as is the design of sampling strategies (possibly with look-ahead) for a more informed expansion of the search space.

%A more immediate direction comes from the observation that the expanding of the AND-OR tree could be more informed: rather than branching on any of the possible outcomes, we could design sampling strategies (possibly with look-ahead) that determine the probabilistically interesting ones. Clearly, this would not compromise the correctness guarantees and would leverage the probabilities to temper the search space.


==> sec-experiments.tex <==
% !TEX root = main.tex

\section{Appendix: Experiments}

\subsection{BridgeWalk}

\emph{(Description of BridgeWalk, as in the dissertation)}

This environment demonstrates that our planner fulfills desideratum~(1): {\sc Pandor} is capable of synthesizing controllers that are less then perfect but whose $\LGT$ exceeds the user-defined $\LGTdesired$ parameter.

% \subsection{Bridge-Plus}

\subsection{Noisy Hall-A}

Our Noisy Hall-A domains are the noisy versions of the Hall-A problems from \citep{Bonet2009-Automatic-derivation}, which came in two variants. The one-dimensional case is shown in Fig.~\ref{fig:probhall-a-one}: the environment is a $1\times n$ grid world, the initial state in the leftmost cell $A$, and the goal is to visit the rightmost cell $B$ and go back to $A$. The observation is $A$ and $B$ in the two end states, and $-$~in the other cells. In our version, both actions (left, right) are noisy in every cell: with $0.5$ probability, the state changes as expected, otherwise the state is unchanged. (State also remains unchanged when moving against the boundary of the environment.)

This planning problem demonstrates that our planner fulfills desiderata (2) and~(3).

The controller synthesized by \citet{Bonet2009-Automatic-derivation}
 was the following:

\centerline{
\begin{tikzpicture}[myautomata]
\fontsize{8}{8}\selectfont
\node[state] (q0) {$q_0$};
\node[state,right=of q0] (q1) {$q_1$};
\draw (q0) edge[loop left] node[align=center] {$A/\rightarrow$ \\ $- / \rightarrow$} (q0);
\draw (q0) edge[->] node[above] {$B/\leftarrow$} (q1);
\draw (q1) edge[loop right] node {$- / \leftarrow$} (q1);
\end{tikzpicture}
}

\noindent They claimed that their
``controllers generalize to Halls of any dimension, and work also in the presence of noise in both the initial situation and in the action effects.''
This statement is true when only the middle cells are noisy, but the controller is inadequate when cell $B$ is noisy as well, because the controller state is changed upon that observation. The controller synthesized by our planner contains the additional edge $q_1 \xrightarrow{B / \leftarrow} q_1$.

The other variant is Halls-A($n \times n$).

{\obeylines
TODO:
 - by favorably ordering the possible actions (and limiting it to two in every state), Pandor solved it in $4.6$~seconds.
 - resulting controller: figure
 - Pandor couldn't solve the 4x4 instance of the problem in 10k seconds
 - Our implementation of HG wasn't able to find a 4-state controller or prove that no 3-state one exists, when all 4 actions were stated as legal on the not-noisy Halls-A(4x4), in an hour.
}

\begin{table}\centering
\begin{tabular}{lrrrcc}
\toprule
Domain & Inst. & $N$ & Time & HG & Fig. \\ % & LTERPCdesired, LTERPC, Works for
\midrule
BridgeWalk & $100$ & $2$ & $0.8$ & HG? & Fig? \\
Noisy Hall-A & $1 \times 4$ & 2 & time? & \Large $\times$ & \ref{fig:probhall-a-one} \\
& $4\times 4$ & N? & time? & \Large $\times$ & Fig? \\
\bottomrule
\end{tabular}
\caption{Summary of experimental results. Column ``HG'' refers to the time for our implementation of \citep{Hu2013-and-or} to solve the problem, with {\Large $\times$} if it wasn't able to.}\label{tab:results}
\end{table}


==> tikz-probhall-a-one.tex <==
\def\x{10mm}

\begin{scope}
    \draw[help lines] (0,0) grid[step=\x] (\x*5,\x);
\end{scope}

\tikzset{every circle/.style={radius=0.5mm}}

\begin{scope}[xshift=\x/2,yshift=.5*\x]

    \node[below] at (0,0) {\bf A};
    \node[below] at (4*\x,0) {\bf B};

    \foreach \i in {0,...,4}
        \draw[fill] (\x*\i,0) circle;

    \def\a{1mm}
    \def\b{4.5mm}

    \begin{scope}[xshift=0*\x,->]
        % \draw (-\a,0) to (-\b,0);
        \draw (180:\a) .. controls +(180:\b) and +(140:\b) .. (140:\a);
        \draw (\a,0) to (\b,0);
        \draw (0:\a) .. controls +(0:\b) and +(40:\b) .. (40:\a);
    \end{scope}

    \foreach \i in {1,2,3} { \begin{scope}[xshift=\i*\x,->]
        \draw (-\a,0) to (-\b,0);
        \draw (180:\a) .. controls +(180:\b) and +(140:\b) .. (140:\a);
        \draw (\a,0) to (\b,0);
        \draw (0:\a) .. controls +(0:\b) and +(40:\b) .. (40:\a);
    \end{scope} }

    \begin{scope}[xshift=4*\x,->]
        \draw (-\a,0) to (-\b,0);
        \draw (180:\a) .. controls +(180:\b) and +(140:\b) .. (140:\a);
        % \draw (\a,0) to (\b,0);
        \draw (0:\a) .. controls +(0:\b) and +(40:\b) .. (40:\a);
    \end{scope}

\end{scope}

\begin{scope}[yshift=-25mm]

    \node[state,initial] at (\x,0) (q0) {$q_0$};
    \node[state] at (4*\x,0) (q1) {$q_1$};

    \draw[->] (q0) edge[loop above] node[align=center] {$A / \rightarrow$\\$- / \rightarrow$} (q0);
    \draw[->] (q0) edge[bend left=10] node[above] {$B / \leftarrow$} (q1);
    \draw[->] (q1) edge[loop above] node {$- / \leftarrow$} (q1);
    \draw[->] (q1) edge[bend left=10] node[below,align=left] {$B / \leftarrow$\\$A / \Xstop$} (q0);

\end{scope}

